StyleTex: Style Image-Guided Texture Generation for 3D Models

Style-guided texture generation aims to generate a texture that is harmonious with both the style of the reference image and the geometry of the input mesh, given a reference style image and a 3D mesh with its text description. Although diffusion-based 3D texture generation methods, such as distillation sampling, have numerous promising applications in stylized games and films, it requires addressing two challenges: 1) decouple style and content completely from the reference image for 3D models, and 2) align the generated texture with the color tone, style of the reference image, and the given text prompt. To this end, we introduce StyleTex, an innovative diffusion-model-based framework for creating stylized textures for 3D models. Our key insight is to decouple style information from the reference image while disregarding content in diffusion-based distillation sampling. Specifically, given a reference image, we first decompose its style feature from the image CLIP embedding by subtracting the embedding's orthogonal projection in the direction of the content feature, which is represented by a text CLIP embedding. Our novel approach to disentangling the reference image's style and content information allows us to generate distinct style and content features. We then inject the style feature into the cross-attention mechanism to incorporate it into the generation process, while utilizing the content feature as a negative prompt to further dissociate content information. Finally, we incorporate these strategies into StyleTex to obtain stylized textures. The resulting textures generated by StyleTex retain the style of the reference image, while also aligning with the text prompts and intrinsic details of the given 3D mesh. Quantitative and qualitative experiments show that our method outperforms existing baseline methods by a significant margin.

==> section/4_experiment.tex <==
\section{Experiments}
\subsection{Implementation Details}
\subsection{Qualitive Results}
\subsection{Comparison to Previous Methods}
\subsection{Ablation Study}
\subsection{Runtime Analysis}
\begin{figure}
  \includegraphics[width=0.99\linewidth]{figure/SDS_ISM_template.pdf}
  \caption{Ablation on ISM loss}
  \label{fig:SDS_ISM}
\end{figure}

\begin{figure*}
  \includegraphics[width=\textwidth]{figure/ablation_tempelate.pdf}
  \caption{Ablation}
  \label{fig:ablation}
\end{figure*}



\begin{figure*}
  \includegraphics[width=\textwidth]{figure/comparison.pdf}
  \caption{Comparison}
  \label{fig:comparison}
\end{figure*}





==> section/4_implementation.tex <==
\section{Implementation Details}
Our texture generation pipeline is developed in Threestudio~\cite{threestudio2023} with Stable Diffusion 1.5~\cite{rombach2021highresolution}. Our evaluation dataset includes 100 3D models, meticulously curated from Objaverse~\cite{deitke2023objaverse} and Sketchfab~\cite{Sketchfab}. The stylistic images for our experiments are derived from the internet or algorithmically generated by Stable Diffusion. The content text prompts for these style images are obtained via GPT-4~\cite{}. We optimize the texture field for 2500 iterations using an Adam optimizer with a leaning rate of 0.005. During the optimization phase, we employ the pre-trained depth and normal ControlNet~\cite{zhang2023adding} to ensure the alignment of the texture details with the geometry of the input mesh. Both the depth map and normal map are rendered in camera space and subsequently normalized to adhere to ScanNet’s standards~\cite{dai2017scannet}. The hyperparameters $\lambda_{cfg}$ and $\lambda_{style}$ in Eq. \ref{eq: final} are set as xxx and xxx. The impact of varying $\lambda_{style}$ values on our results will be elaborated upon in the supplementary materials. The entire optimization process is executed on an NVIDIA RTX 3090 GPU, culminating in approximately xxx minutes.

The optimization of $\Gamma_\theta$ is conducted through the ISM loss during the generative phase. 
%To ensure the textures' storability, editability, and applicability across various rendering platforms, we transform the texture field into a texture map in the post-processing process. 
After obtaining the optimized texture field, we employ a post-processing procedure to ensure the storability, editability, and applicability of the textures across various rendering platforms by transforming the texture field into a texture map with a resolution of $1024^2$. Specifically, similar to ~\cite{Munkberg_2022_CVPR, Chen_2023_ICCV}, we sample the texture field using either the model's inherent UV map or one automatically generated by xatlas~\cite{young2021jpcy}. Furthermore, we apply the UV edge padding technique to fill in the empty regions between UV islands, effectively eliminating unwanted seams.
